Exploration into Translation-Equivariant Image Quantization

This is an exploratory study that discovers the current image quantization (vector quantization) do not satisfy translation equivariance in the quantized space due to aliasing. Instead of focusing on anti-aliasing, we propose a simple yet effective way to achieve translation-equivariant image quantization by enforcing orthogonality among the codebook embeddings. To explore the advantages of translation-equivariant image quantization, we conduct three proof-of-concept experiments with a carefully controlled dataset: (1) text-to-image generation, where the quantized image indices are the target to predict, (2) image-to-text generation, where the quantized image indices are given as a condition, (3) using a smaller training set to analyze sample efficiency. From the strictly controlled experiments, we empirically verify that the translation-equivariant image quantizer improves not only sample efficiency but also the accuracy over VQGAN up to +11.9% in text-to-image generation and +3.9% in image-to-text generation.

==> tab/code_usage.tex <==
\begin{table}[ht]
     \footnotesize
    %\vspace{-5mm}
    \centering
    \caption{The number of codes actually used.% The downsampling method is SC and the codebook size is 256.
    }
    \begin{tabular}{ccc}
         \hline
         Dataset & VQGAN & TE-VQGAN (Ours)  \\
         \hline
         MNIST   & 252 & 14 \\  %($\downarrow$94.4\%)
         FASHION & 250 & 18  \\ %($\downarrow$92.8\%)
         \hline
    \end{tabular}
    \label{tab:code_usage}
    %\vspace{-5mm}
\end{table}

==> tab/img_digit_acc.tex <==
\begin{table*}[ht]
%\vspace{-5mm}
\caption{Digit accuracy of text-to-image generation. %(\textbf{Bold-face} means it outperforms all others statistically significantly.)
}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc|cccc}
\hline
              & \multicolumn{4}{c|}{Seen}                                     & \multicolumn{4}{c}{Unseen}                                    \\ \hline
Model         & Quad1         & Quad2         & Quad3         & Quad4         & Quad1         & Quad2         & Quad3         & Quad4         \\ \hline
MB            & 0.939 (0.023) & 0.931 (0.025) & 0.924 (0.026) & 0.932 (0.025) & 0.724 (0.033) & 0.697 (0.066) & 0.635 (0.067) & 0.620 (0.077) \\
MP            & 0.935 (0.011) & 0.944 (0.008) & 0.942 (0.005) & 0.936 (0.006) & 0.713 (0.007) & 0.703 (0.015) & 0.669 (0.017) & 0.656 (0.028) \\
CB            & 0.942 (0.012) & 0.948 (0.010) & 0.938 (0.012) & 0.937 (0.003) & 0.753 (0.037) & 0.741 (0.034) & 0.682 (0.043) & 0.649 (0.055) \\
SC            & 0.926 (0.011) & 0.926 (0.015) & 0.924 (0.004) & 0.926 (0.011) & 0.812 (0.032) & 0.806 (0.030) & 0.790 (0.038) & 0.761 (0.051) \\
%SC\_emb       & 0.914 (0.002) & 0.923 (0.012) & 0.919 (0.006) & 0.908 (0.002) & 0.810 (0.008) & 0.773 (0.017) & 0.763 (0.036) & 0.732 (0.052) \\
SC\_TE (ours) & \textbf{0.955} (0.013) & \textbf{0.955} (0.007) & \textbf{0.954} (0.013) & \textbf{0.949} (0.011) & \textbf{0.931} (0.033) & \textbf{0.913} (0.032) & \textbf{0.890} (0.048) & \textbf{0.868} (0.059) \\ \hline
\end{tabular}
}
\label{tab:img_digit_acc}
%\vspace{-5mm}
\end{table*}

==> tab/recon_loss.tex <==
\begin{table}[ht]
\footnotesize
%\vspace{-5mm}
\centering
\caption{Reconstruction loss and perceptual loss.}
%\resizebox{\linewidth}{!}{
\begin{tabular}{c|cc|cc}
\hline
        & \multicolumn{2}{c|}{Recon loss}          & \multicolumn{2}{c}{Perceptual loss}      \\ \cline{2-5} 
Dataset & VQGAN & TE-VQGAN     & VQGAN & TE-VQGAN     \\ 
\hline
MNIST   & 0.0079                      & 0.0084 & 0.0036                      & 0.0048 \\
FASHION & 0.0150                      & 0.0187 & 0.0108                      & 0.0198 \\ 
\hline
\end{tabular}
%}
\label{tab:recon_loss}
%\vspace{-5mm}
\end{table}


==> tab/text_digit_acc.tex <==
\begin{table*}[ht]
%\vspace{-5mm}
\caption{Digit accuracy of image-to-text generation.}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc|cccc}
\hline
              & \multicolumn{4}{c|}{Seen}                                     & \multicolumn{4}{c}{Unseen}                                    \\ \hline
Model         & Quad1         & Quad2         & Quad3         & Quad4         & Quad1         & Quad2         & Quad3         & Quad4         \\ \hline
MB            & 0.991 (0.004) & \textbf{0.995} (0.002) & \textbf{0.993} (0.001) & 0.992 (0.002) & 0.587 (0.032) & 0.507 (0.021) & 0.433 (0.013) & 0.378 (0.020) \\
MP            & 0.991 (0.002) & 0.992 (0.003) & 0.990 (0.003) & \textbf{0.993} (0.001) & 0.561 (0.042) & 0.500 (0.038) & 0.412 (0.034) & 0.360 (0.039) \\
CB            & \textbf{0.994} (0.002) & 0.992 (0.002) & 0.992 (0.003) & \textbf{0.993} (0.001) & 0.563 (0.041) & 0.455 (0.056) & 0.362 (0.046) & 0.309 (0.043) \\
SC            & \textbf{0.994} (0.002) & 0.990 (0.001) & 0.989 (0.003) & 0.990 (0.003) & 0.786 (0.052) & 0.692 (0.063) & 0.595 (0.086) & 0.542 (0.106) \\
%SC\_emb       & 0.995 (0.005) & 0.992 (0.001) & 0.991 (0.003) & 0.991 (0.002) & 0.883 (0.011) & 0.775 (0.018) & 0.702 (0.004) & 0.658 (0.011) \\
SC\_TE (ours) & 0.990 (0.007) & 0.987 (0.004) & 0.987 (0.001) & 0.989 (0.001) & \textbf{0.825} (0.037) & \textbf{0.713} (0.066) & \textbf{0.621} (0.061) & \textbf{0.554} (0.065) \\ \hline
\end{tabular}
}
\label{tab:text_digit_acc}
%\vspace{-5mm}
\end{table*}
